Sphere boundaries of hyperbolic groups

We show that a one-ended simply connected at infinity hyperbolic group $G$ with enough codimension-1 surface subgroups has $\partial G \cong \mathbb{S}^2$. Combined with a result of Markovic, our result gives a new characterization of virtually fundamental groups of hyperbolic 3-manifolds. Keywords: CAT(0) cube complexes, Hyperbolic groups, hyperbolic 3-manifolds.

==> disconnection.tex <==
% !TeX root = main.tex

\section{Finding points with different parities}

\begin{enumerate}
\item Existence of $\theta_0$ and $\theta_1$
\item Given a curve and a hyperplane $h$ $\exists \varepsilon$-polygonal approximation which is transverse to $h$.

\begin{lemma}
Let $\crv{C}$ be a simple close curve and $\hyp{h}$ be a hyperplane. For every $\varepsilon>0$, there exists an $\varepsilon$-polygonal approximation of $\crv{C}$ that does not intersect $\hyp{h}$ at a vertex. \todo{definition of $\varepsilon$-polygonal approximation, vertex of an approximation}
\end{lemma}

\begin{lemma}
Let  $\crv{P}$ be a polygonal path and $\hyp{h}$ a hyperplane that does not intersect $\crv{P}$ on a vertex. There exists $\varepsilon>0$ such that for any arc $\arc{k}$ of $\crv{P}$ included in an hyperplane $\hyp{k}$ and any two points $x$ and $y$ of $\hyp{h}$ in an $\varepsilon$-neighborhood of $\arc{k}$, the two point $x$ and $y$ have same parity with respect to $\crv{P}$ if and only if they have same parity with respect to $\hyp{k}$.
\end{lemma}

\begin{corollary}

\end{corollary}
No tangency ? \todo{uses the 2 intersections condition?}

\item Repeat Jordan's proof
\end{enumerate}
